Exploiting Correlation to Achieve Faster Learning Rates in Low-Rank Preference Bandits

We introduce the \emph{Correlated Preference Bandits} problem with random utility-based choice models (RUMs), where the goal is to identify the best item from a given pool of $n$ items through online subsetwise preference feedback. We investigate whether models with a simple correlation structure, e.g. low rank, can result in faster learning rates. While we show that the problem can be impossible to solve for the general `low rank' choice models, faster learning rates can be attained assuming more structured item correlations. In particular, we introduce a new class of \emph{Block-Rank} based RUM model, where the best item is shown to be $(\epsilon,\delta)$-PAC learnable with only $O(r \epsilon^{-2} \log(n/\delta))$ samples. This improves on the standard sample complexity bound of $\tilde{O}(n\epsilon^{-2} \log(1/\delta))$ known for the usual learning algorithms which might not exploit the item-correlations ($r \ll n$). We complement the above sample complexity with a matching lower bound (up to logarithmic factors), justifying the tightness of our analysis. Surprisingly, we also show a lower bound of $\Omega(n\epsilon^{-2}\log(1/\delta))$ when the learner is forced to play just duels instead of larger subsetwise queries. Further, we extend the results to a more general `\emph{noisy Block-Rank}' model, which ensures robustness of our techniques. Overall, our results justify the advantage of playing subsetwise queries over pairwise preferences $(k=2)$, we show the latter provably fails to exploit correlation.

==> noisy-corr.tex <==
\subsection{Lemmas for Almost Independent Random Variables}

This section establishes win probability for pairs/triples consisting of arms from distinct clusters. Here we use $\|\cdot\|_{\rm TV}$ to denote the total variation distance between a pair of random variables. Furthermore, recall that for any pair of random variables $Z_1,Z_2$ defined over a common probability space $\Omega$, the total variation distance acan be expressed as 
\begin{equation}			\label{eqn:def-tv}
\|Z_1 - Z_2\|_{\rm TV} = \sup_{S \subset \Omega} \left|\Pr_{Z_1}(S) - \Pr_{Z_2}(S)\right| 
\end{equation}
Finally, we also recall that mutual information can be expressed as KL divergence between the joint distribution and product measure i.e., $I(X;Y) = D_{\rm KL}(P_{XY} || P_X \otimes P_Y)$.  

\begin{lem}				\label{lem:cross-pb1}
	Let $(\zeta_1,\zeta_2,\zeta_3)$ be jointly distributed with measure $\nu$. Furthermore, suppose we have $I(\zeta;\zeta_2,\zeta_3) \leq \eta$ and  $I(\zeta_2,\zeta_3) \leq \eta$. Then,
	\[
	\Pr_{\nu}\left(\zeta_1 \geq \max(\zeta_2,\zeta_3)\right) \geq \Pr_{\nu_1 \otimes \nu_2 \otimes \nu_3}\left(\zeta_1 \geq \max(\zeta_2,\zeta_3)\right) - O(\sqrt{\eta}) 
	\]
	Furthermore, if the marginals $\nu_1,\nu_2,\nu_3$ are identical, then
	\[
	\Pr_{\nu}\left(\zeta_1 \geq \max(\zeta_2,\zeta_3)\right) \geq \frac13 -  O(\sqrt{\eta}) 
	\]
\end{lem}
\begin{proof}
	Clearly the second part of the lemma follows directly from the first part, hence we shall focus on proving the former. We introduce some additional notation used in the proof. Let $\nu_{23}$ denote the measure corresponding to the joint distribution on $(\zeta_2,\zeta_3)$. Furthermore, given measures $\nu',\nu''$ we use $\nu' \otimes \nu''$ to denote the corresponding product measure. We begin by observing that we can bound
	\begin{align}				
	&\left|\Pr_{\nu} \left(\zeta_1 \geq \max\{\zeta_2,\zeta_3\}\right) - \Pr_{\nu_1 \otimes \nu_{23}} \left(\zeta_1 \geq \max\{\zeta_2,\zeta_3\}\right)
	\right|     \label{eqn:diff1} \\
	&\oleq{1} \left\| \nu - \nu_1 \otimes \nu_{23}\right\|_{\rm TV} \\
	&\oleq{2} \sqrt{D_{\rm KL}\left( \nu || \nu_1 \otimes \nu_{23}\right)} = \sqrt{I(\zeta_1;\zeta_2,\zeta_3)} \leq \sqrt{\eta},			
	\end{align}
	where inequality $1$ is using the definition of $\|\cdot\|_{\rm TV}$ (see \eqref{eqn:def-tv}) and step $2$ is using Pinsker's inequality.
	Now for a fixed $x$, using identical steps we observe that 
	\begin{align}
	\left|\Pr_{\nu_{23}} \left(\zeta_2,\zeta_3 \leq x\right) - \Pr_{\nu_2 \otimes \nu_3} \left(\zeta_2,\zeta_3 \leq x\right) \right| 
	&\leq \left\|\nu_{23} - \nu_2 \otimes \nu_3 \right\|_{\rm TV} \\
	&\leq \sqrt{D_{\rm KL}\left(\nu_{23} || \nu_2 \otimes \nu_3 \right)} = \sqrt{I(\zeta_2;\zeta_3)} \leq \sqrt{\eta}
	\end{align}
	Using the above estimate, we have
	\begin{align*}
	\Pr_{\nu_1 \otimes \nu_{23}} \left(\zeta_1 \geq \max\left(\zeta_2,\zeta_3\right)\right) 
	& = \int^\infty_{- \infty} f_{\nu_1}(\zeta_1) \Pr_{\nu_{23}} \left(\zeta_2,\zeta_3 \leq \zeta_1\right) d{\zeta_1}\\
	& \geq  \int^\infty_{- \infty} f_{\nu_1}(\zeta_1) \Pr_{\nu_2 \otimes \nu_3} \left(\zeta_2,\zeta_3 \leq \zeta_1\right) d{\zeta_1} - \sqrt{\eta} \\
	& =  \Pr_{\nu_1 \otimes \nu_2 \otimes \nu_3} \left(\zeta_1 \geq \max\left(\zeta_2,\zeta_3\right)\right) - \sqrt{\eta} 
	\end{align*}
	Therefore, plugging in the above bound into \eqref{eqn:diff1} we get that 
	\begin{align*}
	\Pr_{\nu} \left(\zeta_1 \geq \max\{\zeta_2,\zeta_3\}\right) 
	&\geq \Pr_{\nu_1 \otimes \nu_{23}} \left(\zeta_1 \geq \max\{\zeta_2,\zeta_3\} \right) - \sqrt{\eta} \\
	&\geq \Pr_{\nu_1 \otimes \nu_2 \otimes \nu_3} \left(\zeta_1 \geq \max\{\zeta_2,\zeta_3\} \right) - 2\sqrt{\eta} 
	\end{align*}
\end{proof}	
	
	Using identical arguments as above we can prove the following.
	\begin{lem}				\label{lem:cross-pb2}
		Let $(\zeta_1,\zeta_2)$ be jointly distributed with measure $\nu$ with identical marginals $\nu_1$ and $\nu_2$. Furthermore, suppose we have $I(\zeta_1;\zeta_2) \leq \eta$. Then,
		\[
		\Pr_{\nu}\left(\zeta_1 \geq \zeta_2\right) \geq \frac12 - O(\sqrt{\eta}) 
		\]
	\end{lem}
	
\subsection{Almost Correlated Random Variables}

\begin{lem}				\label{lem:corr-conc}
	Let $X,Y$ be $(1-\eta)$-correlated identically distributed random variables with $\E[X] = \E[Y] = 0$ and $\E[X^2] = \E[Y^2]  = 1$. Then 
	\[
	\Pr\left(|X - Y| \geq \eta^{1/4}\right) \leq \sqrt{\eta}
	\]
\end{lem}
\begin{proof}
	We begin by observing that due to the first and second moment constraints we have $\E[XY] = {\rm Corr}(X,Y) = 1 - \eta$. Then we can bound the second moment of the random variable $|X-Y|$ as
	\[
	\E\left[(X-Y)^2\right] = \E[X^2] + \E[Y^2] - 2\E[XY] \leq 2 - 2(1 - \eta) \leq 2 \eta.
	\]
	Hence using Markov's inequality we get that
	\[
	\Pr\left(|X - Y| \geq \alpha\right) \leq \Pr\left(|X - Y|^2 \geq \alpha^2\right) \leq \frac{\E\left[|X-Y|^2\right]}{\alpha^2} \leq \frac{2\eta}{\alpha^2}.
	\]
	Setting $\alpha = \sqrt{\eta}$ in the above completes the proof.
\end{proof}

\subsection{Lemmas for Pre-processing}


\begin{lem}				\label{lem:noisy-win}
	Given any triple $\cT:= (1,i,j)$ we  have $\Pr\left(1 | \cT\right) \geq 1/3 - O(\sqrt{\eta})$. 
\end{lem}

\begin{proof}
	The proof consists of several cases depending on the block memberships of $i,j$.
	
	{\bf Case (i)}. Suppose $i,j \in \cB_1$. In this case we note that ${\rm Corr}(\zeta_a,\zeta_b) \geq 1 - \eta$ for any $a,b \in \{1,i,j\}$. We claim that
	\begin{equation}					\label{eqn:imply}
	\Big\{\zeta_1 > \max(\zeta_i - \eta^{1/4}, \zeta_j - \eta^{1/4})\Big\} \Rightarrow \Big\{X_1 > \max(X_i,X_j)\Big\}.
	\end{equation}
	To see this observe that if $\zeta_1 \geq \zeta_i - \eta^{1/4}$ then,
	\[
	X_i  = \mu_i + \zeta_i \overset{1}{<} \mu_i + \zeta_1 + \eta^{1/4} \oleq{2} \mu_1 + \zeta_1 - \eta^{1/4} \leq \mu_1 + \zeta_1 = X_1,
	\]
	where step $1$ is using $\zeta_i < \zeta_1 + \eta^{1/4}$ and step $2$ uses the fact that $\mu_1 \geq \mu_i + 2\eta^{1/4}$. Using identical arguments we can also show that $X_1 > X_j$, which establishes \eqref{eqn:imply}. Therefore, using the contrapositive of \eqref{eqn:imply} we get that 
	\begin{align*}
	\Pr_{X_1,X_i,X_j} \left(X_1 \leq \max(X_i,X_j)\right)
	&\leq \Pr_{\zeta_1,\zeta_i,\zeta_j}\left(\zeta_1 \leq \max\left(\zeta_i - \eta^{1/4} , \zeta_j - \eta^{1/4}\right)\right)  \\
	&\leq \Pr_{\zeta_1,\zeta_i}\left(\zeta_1 < \zeta_j - \eta^{1/4}\right) + \Pr_{\zeta,\zeta_j}\left(\zeta_1 < \zeta_j - \eta^{1/4}\right) \\
	&\leq 4\sqrt{\eta}.
	\end{align*}
	where in the last step we use Lemma \ref{lem:corr-conc} on both terms. Therefore, with probability at least $1 - 4 \sqrt{\eta}$ we have $X_1 > \max(X_i,X_j)$.
	
	{\bf Case (ii)} Suppose $i \in \cB_1$ and $j \in \cB_a$ for some $a \neq 1$. Then as in the previous case, since ${\rm Corr}(\zeta_1,\zeta_i) \geq 1- \eta$ 
	we have $\Pr(X_1 > X_i) \geq 1 - 2\sqrt{\eta}$. Furthermore, since $I(\zeta_1;\zeta_j) \leq \eta$ and $\mu_1 \geq \mu_j$, we have 
	\[
	\Pr_{X_1,X_j}\left(X_1 > X_j\right) \geq \Pr_{\zeta_1,\zeta_j} \left(\zeta_1 > \zeta_j\right) \geq \frac12 - \sqrt{\eta},
	\]
	where the last step follows using Lemma \ref{lem:cross-pb2}. Therefore, by union bound we have 
	\[
	\Pr_{X_1,X_i,X_j}\left( X_1 \leq \max\left(X_i,X_j\right)\right)
	\leq \Pr_{X_1,X_i} \left(X_1 \leq X_i\right) + \Pr_{X_1,X_j} \left(X_1 \leq X_j\right) \leq \frac12 + \sqrt{\eta} + 2\sqrt{\eta} \leq \frac12 + 3\sqrt{\eta}.
	\]	
	
	{\bf Case (iii)} Suppose $i,j \in \cB_a$ for some $a \neq 1$. Here we have $I(\zeta_1;\zeta_i), I(\zeta_1;\zeta_j) \leq \eta$ and ${\rm Corr}(\zeta_i,\zeta_j) \geq 1 - \eta$. Without loss of generality, assume that $\mu_i \geq \mu_j$. Since $I(\zeta_1;\zeta_i) \leq \eta$, using Lemma \ref{lem:cross-pb2} we have 
	\begin{equation}					\label{eqn:event1}
	\Pr_{\zeta_1,\zeta_i} \left(\zeta_1 \geq \zeta_i\right) \geq \frac12 - \sqrt{\eta}.
	\end{equation}	
	Furthermore, since ${\rm Corr}(\zeta_i,\zeta_j) \geq 1 - \eta$, using Lemma \ref{lem:corr-conc}
	\begin{equation}					\label{eqn:event2}
	\Pr_{\zeta_i,\zeta_j} \left(\zeta_j \leq \zeta_i + \eta^{1/4}\right) \geq 1 - 2\sqrt{\eta}.
	\end{equation}
	We claim that conditioned on these event in probability expressions in \eqref{eqn:event1} and \eqref{eqn:event2} we have $X_1 > \max(X_i,X_j)$ with probability $1$. Indeed, using the event in \eqref{eqn:event1} and $\mu_1 > \mu_i$ we have $X_1 = \mu_1 + \zeta_1 > \mu_i + \zeta_i = X_i$. Furthermore, 
	\[
	X_j = \mu_j + \zeta_j \oleq{\eqref{eqn:event2}} \mu_i + \zeta_j + \eta^{1/4} \leq \mu_1 + \zeta_i  \overset{\eqref{eqn:event1}}{<} \mu_1 + \zeta_1 = X_1,
	\]
	where the middle inequality again uses $\mu_1 \geq \mu_j + 2\eta^{1/4}$ in our setting. Therefore, combining the above observation with the bounds from \eqref{eqn:event1},\eqref{eqn:event2} we get that
	\[
	\Pr_{X_1,X_i,X_j}\left(X_1 > \max(X_i,X_j)\right) 
	\geq \Pr_{\zeta_1,\zeta_i,\zeta_j}\left(\{\zeta_1 \geq \zeta_i\} \wedge \{\zeta_j \leq \zeta_i + \eta^{1/4}\}\right)
	\geq \frac12 - 3\sqrt{\eta}.
	\]
	
	{\bf Case (iv)} Suppose $i \in \cB_a$ and $j \in \cB_b$ where $a \neq b$ and $a,b \neq 1$ i.e., the arms $1,i,j$ belong to distinct blocks. Then using Lemma \ref{lem:cross-pb1} we have 
	\[
	\Pr_{\zeta_1,\zeta_i,\zeta_j}\left(\zeta_1 \leq \max(\zeta_i,\zeta_j)\right) \geq \frac13 - 4\sqrt{\eta}.
	\]
	Since $\mu_1 \geq \mu_i,\mu_j$, we have 
	\[
	\Pr_{X_1,X_i,X_j} \left(X_1 \geq \max(X_i,X_j)\right) \geq \Pr_{\zeta_1,\zeta_i,\zeta_j}\left(\zeta_1 \leq \max(\zeta_i,\zeta_j)\right) \geq \frac13 - 4\sqrt{\eta}.
	\]
	
\end{proof}

The above follows directly from Case (iii) of the above lemma.

\begin{cor}			\label{corr:cross-win}
	Given a triple $\cT = (1,i,j)$ where $i,j \in \cB_a$, we have that $\Pr\left(\{j,k\}| \cT\right) \leq \frac12 + O(\sqrt{\eta})$.
\end{cor}


\subsection{Analysis of the Pre-processing Step}

\blue{Non-noisy analysis}

The following observation on directed graphs is going to be useful.

\begin{obs}			\label{obs:graph}
	Let $G = (V,E)$ be a complete directed graph on $n$-vertices. Then, there can be at most one vertex $i \in V$ such that $\text{in-deg}(i) = 0$, where $\text{in-deg}(\cdot)$ denotes the in-degree of a vertex.
\end{obs}
\begin{proof}
	For contradiction, suppose there exists two such vertices $i,j$. Then, the orientation of the edge $\{i,j\}$ will enforce $\text{in-deg}(i) > 0$ and 
	$\text{in-deg}(j) > 0$, which gives us a contradiction.
\end{proof}

\begin{lem}
	For every $a \in [r]$ we have $| \cB_a \cap S| \leq 1$.
\end{lem}
\begin{proof}
	Fix a block $\cB_a$. Now consider a triple $(1,i,j)$ where $i,j \in \cB_a$. Then,
	\[
	\min\left(\Pr\left(i|\cT\right),\Pr\left(j|\cT\right)\right) \leq \frac{1}{4} + O(\sqrt{\eta})
	\]
	i.e., at least one of $i,j$ wins with probability at most $1/4 + O(\sqrt{\eta})$. Using this observation, we construct a complete directed graph $G_a = (\cB_a,E_a)$ as follows. The vertex set of the graph is $\cB_a$. For any pair of vertices $i,j$, we add an edge in the following say
	\begin{itemize}
		\item If $\Pr(i | \cT) > 0.26$ and $\Pr(j | \cT) \leq 0.26$, we add an edge $i \to j$.
		\item If $\Pr(i | \cT) \leq 0.26$ and $\Pr(j | \cT) > 0.26$, we add an edge $j \to i$.
		\item If $\Pr(i | \cT), \Pr(j | \cT) \leq 0.26$, we add an edge arbitrarily. 
	\end{itemize}
	Now note that the above graph $G_a$ is a complete directed graph (i.e., a tournament) which satisfies the following property. For every pair of vertices if $\{i,j\} \subseteq \cB_a$ if the edge is oriented from $i$ to $j$ then, when the triple $(1,i,j)$ is played, then $j$ is flagged (this holds since $\Pr(j| \cT) \leq 0.26$ from the construction of $G_a$). Therefore, the set of vertices (arms) eliminated when all triples of the form $(1,i,j)$ are played include the set of vertices $i \in \cB_a$ for which $\text{in-deg}(i) \geq 1$. Since Observation \ref{obs:graph} implies that there can be at most one vertex with $0$ in-degree, it follows that there can be at most one arm which is not flagged, and hence, not eliminated.
\end{proof}

\begin{lem}
	At the end of pre-processing we have $1 \in S$.
\end{lem}
\begin{proof}
	From Lemma \ref{lem:noisy-win}, we know that in any triple $(1,i,j)$, we have $\Pr(1| \cT) \geq 1/3 - O(\sqrt{\eta})$ and hence item $1$ never gets eliminated.
\end{proof}
	




==> rep-alg-proof.tex <==
\subsection{Proof of Theorem \ref{thm:ub_gbr}}

The proof of the theorem mainly goes along the lines of Theorem from \cite{SG20}. The improvement in our sample complexity comes from  which gives improved sample complexity for $\epsilon$-optimal winner determination problem on a fixed subset.

\begin{lem}						\label{lem:rank-conc}
	Let $\mu = (\mu_1,\ldots,\mu_q)$ and $ \Sigma \in \{0,1\}^{q \times q}$ be the {\em distinct} scores and covariance matrix for a fixed set of $q$-arms such that $\mu_1 > \mu_2 \geq \ldots \mu_q$. Let $\brank(\Sigma) = r$. Let $T \subset [q]$ denote the set of $\epsilon$-sub-optimal arms. Suppose $[q]$ is played $t$ times, and let $N_i(t)$ denote the number of times arm $i$ wins. Then, if $t \geq O(r\epsilon^{-2}\log(r/\delta))$, then with probability at least $1  - \delta$ we have 
	\[
	N_t(1) > \max_{i \in T} N_t(i)
	\]
\end{lem}

The proof of the above lemma is based around the following elementary idea: even if a subset has $k$-arms, due to the block rank assumption, the winner determination problem on that subset can essentially be reduced to winner determination on a (at most) $r$-sized subset -- hence it suffices to play subsets $\tilde{O}_\epsilon,\delta(r)$ times instead of the $\tilde{O}_{\epsilon,\delta}(k)$. We defer the proof of the above for now, and complete the analysis of the theorem. As is usual, we complete the analysis in $2$-steps. The first lemma bounds the number of samples queried by the algorithm.

\begin{lem}				\label{lem:samp-comp}
	The sample complexity of the algorithm is $O\left(\frac{nr}{qc^2\epsilon^2}\log\frac{n}{k\delta}\right)$.
\end{lem}
\begin{proof}
	Let $S_{\ell}$ denote the set of item being played in iteration $\ell$ of the outer while loop. Since, going from iteration $\ell$ to $\ell+1$, the algorithm retains exactly $1$ item out of each $k$-sized subset, we have $|S_{\ell + 1}| \leq |S_{\ell}|/k$\footnote{To be precise, the exactly inequality here $|S_{\ell + 1}| \leq |S_{\ell}| + 1$, however, we ignore the additional term for keeping the computation clean, since it does not affect the overall asymptotic estimate.} Therefore, by recurrence we have $|S_{\ell}| \leq n/k^{\ell}$; this implies that the outer while loop can run for at most $\ln k + 1$ iterations. Furthermore, in the $\ell^{th}$ iteration, each $k$-sized subset is played $t_\ell = r\epsilon^{-2}_\ell \log(r/\delta_{\ell})$-times. Combining these observations, we can bound the sample complexity as 
	\begin{align*}
	\sum_{\ell = 1}^{\ln k + 1} \frac{n}{k^{\ell}}\cdot \left(\frac{r}{(3/4)^{2\ell} \epsilon^2c^2} \log \frac{r}{(3/4)^{\ell} \delta}\right)
	&\leq \sum_{\ell = 1}^{\ln k + 1} \frac{n}{k^{\ell}}\cdot \frac{\ell}{(3/4)^{\ell}}\left(\frac{r}{\epsilon^2c^2} \log \frac{r}{\delta}\right) \\
	&\leq \sum_{\ell = 1}^{\ln k + 1} \frac{n}{k^{\lceil\ell/2 \rceil}}\cdot \frac{\ell}{(3/4)^{\ell}}\left(\frac{r}{\epsilon^2c^2} \log \frac{r}{\delta}\right) \\
	&\leq O\left(\frac{nr}{k\epsilon^2c^2} \log \frac{r}{\delta}\right) \\
	\end{align*}
\end{proof}

Now, using lemma \ref{lem:rank-conc}, the following lemma shows that w.p. at least $1 - \delta$. the algorithm the optimal item.

\begin{lem}				\label{lem:win-corr}
	With probability at least $1 - \delta$, over all the iterations $\ell$,  the best item is retained in the set $S_\ell$.
\end{lem}
\begin{proof}
	Clearly, it suffices to bound the probability of the event $1 \notin S_{\ell}$ for some iteration $\ell$. Towards that let $\cG_{\ell}$ be the $k$-sized subset which contains the best item in iteration $\ell$. 
	\begin{align*}
	\Pr\left(\exists \ \ell, 1 \notin S_{\ell}\right)
	&\leq \sum_{\ell = 1}^{\ln k + 1} \Pr\left(1 \notin S_{\ell + 1} \Big| 1 \in S_{\ell - 1}\right) \\
	&\leq \sum_{\ell = 1}^{\ln k + 1} \Pr\left(1 \neq \argmax_{i \in \cG_{\ell}} w_i  \Big| 1 \in S_{\ell - 1}\right) \\
	&\oleq{1} \delta_\ell \leq \sum_{\ell}\delta/2^{\ell} \leq \delta 
	\end{align*}
	where inequality $1$ follows using Lemma \ref{lem:rank-conc}.
\end{proof}

Combining the guarantees of the two lemmas above  completes the proof of Theorem \ref{thm:ub_gbr}.

\subsubsection{Proof of Lemma \ref{lem:rank-conc}}

	For every $i \geq 1$, denote $T_i := T \cap \cB_i$ and without loss of generality, we can assume $T_i \neq \emptyset$ for every $i \in [r]$. Furthermore, define $\sigma(1) = 1$ and for every $i \in [r]\setminus \{1\}$, let $\sigma(i) \in \argmax_{j \in T_i} \mu_j$. Now for every trial $\ell \in [t]$, let $g^{(\ell)}_{\sigma(i)}$ be the realization of noise component of the corresponding arm $\sigma(i)$. Note that since the collection includes at most one arm from each block, the arms corresponding to $\sigma(1),\ldots,\sigma(r)$ are independent. For every $i \in [r]$, we define the cluster win-count $N'_i(t)$ as 
	\[
	N'_i(t) := \left| \left\{ \ell \in [t] : \argmax_{j \in [r]} g^{(\ell)}_{\sigma(j)} + \mu_{\sigma(j)} = i \right\} \right|
	\]  
	It is easy to see that for every $i \in [r]$ we have 
	\[
	N'_1(t) = N_1(t) \qquad\qquad \textnormal{and} \qquad\qquad N'_i(t) = \sum_{j \in T_i} N_j(t), \qquad \forall \ i \in [r] \setminus\{1\}
	\]
	The first equality follows by definition. For the second equality. Observe that any arm $j \in T_i$ wins in a trial $\ell$ if and only if $g^{(\ell)}_{\sigma(i)} + \mu_{\sigma(i)} > g^{(\ell)}_{\sigma(i')} + \mu_{\sigma(i')}$ for every $i'\neq i$. From the above equation, it directly follows that 
	\[
	\left\{N_t(1) < \max_{i \in T} N_t(i)\right\} \Rightarrow \left\{N'_t(1) < \max_{i \in [r] \setminus \{1\}} N'_t(i)\right\}
	\]
	Therefore if suffices to upper bound the probability of the event from the RHS of the above equation, which can be stated equivalently as follows. Given independent arms $\sigma(1),\ldots,\sigma(r)$ with $\mu_{\sigma(1)} - \mu_{\sigma(i)} \geq \epsilon$ for every $i \in [r]$, arm $\sigma(1)$ wins the maximum number of rounds in $t$ trials -- this is at most $\delta$ using Theorem \ref{thm:rum-conc} \blue{cite RUM concentration}.

